Batch Clipping and Adaptive Layerwise Clipping for Differential Private Stochastic Gradient Descent

Each round in Differential Private Stochastic Gradient Descent (DPSGD) transmits a sum of clipped gradients obfuscated with Gaussian noise to a central server which uses this to update a global model which often represents a deep neural network. Since the clipped gradients are computed separately, which we call Individual Clipping (IC), deep neural networks like resnet-18 cannot use Batch Normalization Layers (BNL) which is a crucial component in deep neural networks for achieving a high accuracy. To utilize BNL, we introduce Batch Clipping (BC) where, instead of clipping single gradients as in the orginal DPSGD, we average and clip batches of gradients. Moreover, the model entries of different layers have different sensitivities to the added Gaussian noise. Therefore, Adaptive Layerwise Clipping methods (ALC), where each layer has its own adaptively finetuned clipping constant, have been introduced and studied, but so far without rigorous DP proofs. In this paper, we propose {\em a new ALC and provide rigorous DP proofs for both BC and ALC}. Experiments show that our modified DPSGD with BC and ALC for CIFAR-$10$ with resnet-$18$ converges while DPSGD with IC and ALC does not.

==> Chapters/01_DifferentialPrivacy.tex <==
\chapter{Differential Privacy}
\label{chapter:Differentialprivacy}
\section{What is Privacy?}

At first thought, you may wonder why we need data privacy and what it exactly means. Unfortunately, there is no exact definition for privacy because it depends on the context and what information we consider to be "private." For example, each person has their own different set of private information, such as address, phone number, name, and so on. Hence, this information is considered sensitive data and no one wants this information to be revealed to any other party without their permission. Therefore, Dwork \cite{DPbook} proposed a formal mathematical definition of privacy called Differential Privacy, which assures that there is hardly a behavior change when an individual's data is added to or removed from the dataset.

\section{Differential Privacy}
Let the randomized mechanism $M$ be the algorithm applied by the curator when releasing information, thus we do not need to distinguish interactive setting and non-interactive setting. Moreover, we say the databases $D_1$ and $D_2$ are neighboring databases if they just differ at most one element. 
\begin{definition}
\label{DP:definition}
A randomized mechanism $M$ gives $(\epsilon,\delta)$-differential privacy if for \textbf{all} neighboring databases $D_1$ and $D_2$, and all $S \subseteq Range(F)$:
\[Pr[M(D_1) \in S] \leq e^\epsilon Pr[M(D_2) \in S] + \delta \]
When $\delta = 0$, the guarantee is simply called $\epsilon$-DP
\end{definition}

A mechanism M satisfying this definition can ensure the privacy for any participant data even if he/she either adds his/her data to the database or removes his/her data from the database. For example, the presence or absence of a patient profile in a hospital database does not affects significantly the outcomes of the differential  private mechanism M which is used by that hospital.

Differential privacy provides a very strong guarantee of privacy. To be detailed, it is just a statistical property about the behavior of the randomized mechanism, thus it is independent of the computational power and auxiliary information available to the adversary/attacker. However, Differential privacy does not give absolute guarantee of privacy and we measures the cost as privacy loss given the output $o$ of the mechanism M:
\begin{equation}
    % \begin{aligned}
    PL_{M(D_1)||M(D_2)}^{o} = \ln \left(\frac{Pr[M(D_1) = o]}{Pr[M(D_2) = o]}\right)
    % \end{aligned}
\end{equation}

Dwork and Roth have shown that any $(\epsilon,\delta)-$differentially private mechanism ensures that for all neighboring database $D_1,D_2$, the absolute value of privacy loss will be bounded by $\epsilon$ with probability at least $1 - \delta$.

Next, we introduce the properties of differential privacy which helps it extremely useful and be applicable to solve many privacy problems.
\subsection{Properties}
There are four majors properties of differential privacy which are: Post-processing, Group Privacy, Basic Composition and Advance Composition.
\begin{properties} \textbf{Post-processing:} Let $M: \mathbb{N}^{|X|} \rightarrow R$  be a randomized algorithm that is $(\epsilon,\delta)$-differentially private. Let $f: R \rightarrow R'$ be an arbitrary deterministic mapping. Then $f \circ M : \mathbb{N}^{|X|} \rightarrow R'$ is $(\epsilon,\delta)$-differentially private.
\end{properties}


\begin{properties} \textbf{Group Privacy:} Let $M: \mathbb{N}^{|X|} \rightarrow R$ be a randomized algorithm that is $(\epsilon,\delta)$-differentially private. Then, M is $(k\epsilon,ke^{k-1}\delta)$-differentially  private for groups of size k. That is, for databases $x,y \in \mathbb{N}^{|X|}$ such that $||x=y||_1 \leq k $ and for all $S \subseteq R$ we have:
\[Pr[M(x_1) \in S] \leq e^{k\epsilon} Pr[M(x_2) \in S]  + ke^{k-1}\delta\]
\end{properties}
\begin{properties} \textbf{Basic Composition:} Let $M_i: \mathbb{N}^{|X|} \rightarrow R_i$ be a randomized algorithm that is $(\epsilon_i,\delta_i)$-differentially private for $i = 1,2,3,...,k$. Then, the composition $M_{[k]}: \mathbb{N}^{|X|} \rightarrow R_1 \times R_2 \times \dots \times R_k$ defined as:
\[M_{[k]}(x) = (M_1(x),M_2(x),M_3(x),\dots ,M_k(x))\] is $(\sum_{i=1}^k\epsilon_i,\sum_{i=1}^k\delta_i)$-DP
\end{properties}
\begin{properties} \textbf{Advanced Composition:} Let $M: \mathbb{N}^{|X|} \rightarrow R^K$ a k-fold adaptive composition of $(\epsilon_i,\delta_i)$-DP mechanisms. Then, M is $\epsilon', k\delta + \delta'$-DP for:
\[\epsilon' = \epsilon \sqrt{2k \ln(\frac{1}{\delta'})} + k\epsilon(e^\epsilon -1)\] is $(\sum_{i=1}^k\epsilon_i,\sum_{i=1}^k\delta_i)$-DP
\end{properties}

% \pagebreak % TODO: automatically page break for algorithm

\subsection{Gaussian Mechanism}
Dwork \cite{DPbook} proposed many mechanisms such as Gaussian Mechanism, Laplace Mechanism and Exponential Mechanism which provides the privacy for and function $f$ by adding the Gaussian noise, Laplace noise or choosing the output "randomly" based on the a certain probability, respectively. However, in this work, we only focus on Gaussian Mechanism which is mainly used on our private deep learning training algorithm and DP analysis.

\begin{definition}
\label{def:gaussianmech}
    Let $f: \mathbb{N}^{|X|} \rightarrow R^d$ be an n arbitrary $d$-dimensional function and the $\ell_2$ sensitivity of $f$ be $||f||_2 = max_{x,y} ||f(x)-f(y)||_2$ for any neighboring datasets $x$ and $y$. The Gaussian Mechanism with parameter $\sigma$ adds the $\sigma$ adds the Gaussian noise $N(0,\sigma^2)$ to each of $d$ components of the output. Then with any $\epsilon \in (0,1)$, for $c^2 > 2\ln (1.25/\delta)$, the Gaussian Mechanism with $\sigma \geq c \frac{||f||_2}{\epsilon}  $ is $(\epsilon,\delta)$-differentially private.
\end{definition}

By injecting noise into the datasets, we can perform all possible statistical analyses without identifying any personal sensitive information. Differential Privacy motivates users to share their personal information without worrying about it being exposed by other parties. Therefore, it solves a significant problem for other computer science subjects that rely heavily on user data, such as Internet of Things (IoT) or Machine Learning/Deep Learning. Based on the above analysis, Differential Privacy is an ideal tool to provide privacy for Machine Learning and Deep Learning models, which is a primary topic we have been focusing on.




% \begin{mechanism} 
% \textbf{Gaussian Mechanism:} TBD
% \end{mechanism}
% \begin{mechanism} 
% \textbf{Laplace Mechanism:} TBD
% \end{mechanism}
% \begin{mechanism} 
% \textbf{Exponential Mechanism:} TBD
% \end{mechanism}
% \section{Differential Privacy Variants}
% \begin{definition} Local Differential Privacy (LDP): A randomized algorithm $M$ gives $(\epsilon,\delta)$-differential privacy if for \textbf{all pairs} of user's possible private data $x_1$, $x_2$, and all subsets $S \subseteq Range(M)$:
% \[Pr[M(x_1) \in S] \leq e^\epsilon Pr[M(x_2) \in S] + \delta \]

% \end{definition}
% \subsection{\href{https://arxiv.org/pdf/1702.07476.pdf}{\textcolor{blue}{Renyi Differential Privacy}}}
% \begin{definition}
% \textbf{Renyi Divergence}: For two probability distributions P and Q defined over R (the image of the DP mechanism), the Renyi divergence of order $\alpha > 1$ is 
% \[D_\alpha (P||Q) = \frac{1}{\alpha - 1} \log E_{x \sim Q} (\frac{P(x)}{Q(x)})^\alpha\]
% \end{definition}
% \begin{definition}
% $(\alpha,\epsilon)-$\textbf{RDP}: A randomized mechanism $M:D \rightarrow R$ is said to have  $\epsilon$-Renyi differential privacy of order $\alpha$  if for \textbf{all} data sets $D_1$ and $D_2$ differing only on at most one element, it holds that:
% \[D_\alpha(M(D)||M(D') \leq \epsilon\]
% Or
% \[Pr[M(D) \in S] \leq (e^\epsilon Pr[M(D') \in S])^{\frac{\alpha-1}{\alpha}} \] for any subset $S \subseteq R$
% \end{definition}
% \begin{properties}
% \textbf{Post Processing and Group privacy:} the same as $(\epsilon,\delta)$-DP
% \end{properties}
% \begin{properties}
% \textbf{Basic Composition:} Let $f: D \rightarrow R_1$  be $(\alpha,\epsilon_1)$-RDP and $g: D \rightarrow R_2$  be  $(\alpha,\epsilon_2)$-RDP, then the mechanism defined as (X,Y), where $X \sim f(D)$, $Y \sim g(D)$, satisfies $(\alpha, \epsilon_1 + \epsilon_2)$-RDP
% \end{properties}
% \textbf{Advanced Composition:}:  Let $f: D \rightarrow R$  be an adaptive composition of n mechanisms all satisfying $\epsilon$-RDP. Let D and D' be two adjacent inputs. Then for and $S \subseteq R$:
% \[Pr(f(D) \in S] \leq exp\left(2 \epsilon \sqrt{n \log (1/Pr[f(D') \in S])}\right) \cdot Pr[f(D') \in S]\]
% \textbf{Moment Accountant:} For $\alpha \leq 1 +\sigma^2\ln{\frac{1}{q\sigma}}$, the DPSGD algorithm is $(\alpha, q^2 \frac{\alpha}{(1-q)\sigma^2}+ O(q^3\alpha^3/\sigma^3)$-RDP for $q \rightarrow 0$
% \subsection{RDP versus DP}
% % \begin{figure}[H]
% %     \centering
% %     \includegraphics[scale=0.5]{Differential Privacy/images/RDP_DP.PNG}
% %     \caption{RDP versus DP}
% %     \label{fig:RDP_DP}
% % \end{figure}
% \subsection{\href{https://projects.iq.harvard.edu/files/privacytools/files/bun_mark_composable_.pdf}{\textcolor{blue}{Concentrated Differential Privacy (CDP)}}}
% Let $M_{\alpha}(A, S,S') = exp(\alpha D_{\alpha+1}(A(S)||A(S')))$, 
% The following are equivalent definitions of CDP,zCDP,tCDP and RDP:
% \begin{definition}
% For all adjacent databases S,S', a mechanism A satisfies:
% \begin{itemize}
%     \item $(\mu,\tau)$-CDP if:
%     \[E_{z\sim A(S)} [c(z;A,S,S')] \leq \mu, M_\alpha(A,S,S') \leq exp(\frac{\alpha^2\beta^2}{2})\]. for all $\alpha \geq 1$
%     Where $c(z;A,S,S')$ is the privacy loss of mechanism A given output z.
%     \item $(\xi,\rho)$-zCDP if:
%     \[\forall \alpha > 0: M_\alpha(A,S,S') \leq exp(\alpha(\xi + \rho(\alpha+1)))  \]
%     \item $(\rho,\omega)$-tCDP if:
%     \[\forall \alpha \in (0,\omega): M_\alpha(A,S,S') \leq exp(\rho \alpha(\alpha +1))\]
%     \item $(\alpha,\epsilon)$-RDP if:
%     \[M_{\alpha-1} (A,S,S') \leq exp((\alpha-1)\epsilon)\]
% \end{itemize}
% \end{definition}


% \section{Deep Learning}
% \subsection{Federated Learning}
% % \subsection{Online Learning}

% \section{Differentially Private Training Methods}
% \subsection{Differential Private Stochastic Gradient Descent (DPSGD)}
% TBD: Add intro here


% \begin{definition}

%  \textbf{Moment Accountant \href{https://arxiv.org/pdf/1607.00133.pdf}{(\textcolor{blue}{Deep Learning with Differential Privacy})}:} There exist constants $c_1$ and $c_2$ so that given
% the sampling probability $q = L/N$ and the number of steps
% T, for any $\epsilon < c_1 q^2 T$, the DPSGD algorithm is $(\epsilon,\delta)$-DP for \textbf{any} $\delta > 0$ if we choose:
% \[\sigma \geq c_2 \frac{q\sqrt{T\log{1/\delta}}}{\epsilon}\]

% \end{definition}

==> Chapters/02_DeepLearning.tex <==
\chapter{Deep Learning}
\label{chapter:Deeplearning}

In this chapter, we would like to talk about Deep Learning neural network components as well as how to train these network in order to do specific tasks such as Image Classification, 
\section{Deep Learning}
Deep learning is a subset of machine learning that involves the use of neural networks to learn from data. A neural network is a mathematical model that is designed to simulate the behavior of neurons in the brain. It consists of layers of interconnected nodes, each of which performs a simple mathematical operation on its inputs.

In a deep neural network, there are multiple layers of nodes, allowing the network to learn increasingly complex representations of the data. Each layer in the network transforms the input it receives from the previous layer, eventually producing an output that represents the network's prediction or classification of the input.

Deep learning neural networks have been used to achieve state-of-the-art performance on a wide range of tasks, including image and speech recognition, natural language processing, and game playing. They have also been applied to fields such as finance, healthcare, and transportation, where they are used to identify patterns and make predictions based on large amounts of data.

However, deep learning neural networks require a large amount of data and a good learning method to optimize the neural network's parameters. In this chapter, we will cover a various of learning method for a deep learning model as well as model's architecture for image classification task.

To sum it up, to train a deep learning model, we need to define the model's architecture, optimizer, loss function on a training dataset we want the model to learn about it.
\subsection{Model Architecture}
Since this work only focus on image classification task, we will only talk about Fully Connected Layer, Convolutional Layer, Batch Normalization which we used our differential private training on.
\subsubsection{Neuron (perceptron)}
The neural networks is built based on a set of dependent neurons (or perceptions). In other words, a neuron, is a basic unit in a deep learning neural networks. Mathematically, a neuron is a non-linear function which consists of 4 main parameters: Input values $x$, weights and Bias $w and b$, net sum function and activation function $f$. We have the output of a neuron as:
\[y = f(\sum_{1=1}^{n} w_i x_i + b)\] assuming $x$ and $w$ have $n$ elements/rows

There are many types of Activation functions:
\begin{itemize}
    \item Sigmoid function: $f(x) = \frac{1}{1+e^{-x}}$
    \item Relu: $f(x) = \left\{\begin{array}{lr}
        x, & \textit{for } x \geq 0\\
        0, & \textit{for } x < 0
        \end{array}\right. $
    \item Tanh: $f(x) = \frac{e^x – e^{-x}}{e^x + e^{-x}} $
    \item Sign function: $f(x) = \left\{\begin{array}{lr}
        -1, & \textit{for } x < 0\\
        0, & \textit{for } x = 0 \\
        1, & \textit{for } x \geq 0
        \end{array}\right. $
\end{itemize}

These activation functions is chosen depended on different problems and the desired outputs. Moreover, they may also cause the slow learning process or vanishing gradients or exploding gradients which are very bad effects during the backpropagation process in the training process \cite{ExplodingGradpaper}. 

\subsubsection{Fully Connected Layer}
In fully connected layers, the neurons first perform a linear computation on the input vector though the weights matrix. After that, a non-linear transformation is applied through the activation function $f$. Note that the input of the fully connected layer is flattened into a single vector in order to perform the mentioned computation. Therefore, in fully connected neural networks, all neurons is connected to all neurons in the next layers. On the other hand, this layer also is used as the last layer in the networks and outputs the classification decision which called "softmax" layer:
\[softmax(x)_i = \frac{e^{x_i}}{\sum_{j=1}^{n}e^{x_i}}\]
where $n$ is the number of classes.

\subsubsection{Convolutional Layer}
A convolutional layer performs a convolution operation of the inputs using filters and kernels. This operation is simply sliding each filter over the input data and computing the dot product between the filter and the input data in the kernel. This results in a single scalar value which is a new value of the chosen input data.

Since the filter can only slide over the input data until it reaches the edge, this makes the output of a convolutional layer has smaller dimension than the input data. Moreover, the border pixels are also used less frequently than the center pixels which may cause some information loss while training on the input data. To overcome this problem, the input data is often padded with zeros as the border in order to maintain the size of the feature map and use more information from pixels at the edges. Usually, to do this, the padding size is usually equal to kernel size minus 2.

Similarly to fully connected layer, after the convolution operation, the convolutional layer also applies a non-linear activation function such as ReLu to the output feature maps. This enables the non-linearlity to the network and allows it to learn nmore complex features from the input data.

However, because of the convolution operation, the output of features map can be diverges and makes the model learn slower and may not have good performance. Therefore, in some very deep network such as Resnet-18,Resnet-34,... \cite{resnet18paper}. The batch normalization layer is often used in order to normalize all the output features and thus accelerate the training process of the convolutional neural network. \cite{ioffe2015batch}. 

\subsubsection{Batch Normalization}
In this layer, the input data to this layer is normalized as follows:
\[y = \frac{x-E[x]}{\sqrt{Var[x]+\epsilon}} \times \gamma + \beta\]

The mean and the standard-deviation are calculated per-dimension over the minibatches and $\gamma$, $\beta$ are learnable parameter. By default, $\gamma = 1, \beta = 0$ and will be updated during the training process.

However, Opacus \cite{Opacus}, a popular Differentially private Deep Learning training framework, could not apply this layer because it violates the differential privacy if we do not put a privacy mechaism for this layer. This is because this layer makes each sample's normalized value depend on its peers in a batch which yeild a vioation in DPSGD training algorithm. We will discuss about this problem in chapter \ref{chapter:DPSGD}
\subsection{Optimizer}
Given a loss function, the goal of the neural network training process is minimizing/maximizing the loss function. Therefore, optimizers are used to adjust the model's parameters in order to minimizing/maximizing the loss function. The loss function can be strongly convex, convex, concave,... etc. Depends on type of loss function, there are many optimizers are introduced in order to reach the closest point to the global solution. However, because this works only focus on differentially private stocastic gradient descend algorithm. We will only introduce about gradient descent, Stocastic gradient descend method and minibatch stocastic gradient descent.

Asuming we have the model $w$ and we want to minimize the loss function $L$ with the dataset $D = (x,y)$:
\[ min_{w}\ L(w(x),y)\]
\subsubsection{Gradient Descent}
Gradient descent is one of the most popular method to minimize the loss function of a model. It is a method for finding the optimal values of the parameters in a model by iteratively adjusting them in the direction of the steepest descent of the loss function.

The idea behind gradient descent is to start with an initial set of parameter values, and then repeatedly update them in the direction of the negative gradient of the loss function with respect to the parameters. This means that the parameters are adjusted in the direction that reduces the loss function the most.

The gradient descent algorithm works by computing the gradient of the loss function with respect to each parameter in the model, and then adjusting each parameter by subtracting a small fraction of the gradient (known as the learning rate). This process is repeated for a fixed number of iterations or until the change in the loss function falls below a certain threshold. Let the learning rate is $\eta$, we have the gradient descent update as follow:

\[w \leftarrow w - \eta \nabla_{w} L(w,x)\]

Here, the learning rate $\eta$ plays an important role in minimizing the loss function. If the learning rate is too big, the update will be diverged, i.e. updating $w$ will increase the loss instead of minimize it. On the other hand, if the learning rate is too small, then there will be very small update on $w$, thus leads to slow convergence in the training process and will cost a lot of updates on $w$ to have a good result. Therefore, we use diminising learning rate in our algorithm where we start with a learning rate $\eta_0$ big enough, then decrease it after a certain update iterations. This method not only preventing the diverging problem but also give us better results because we can reach a closer point to the optimal solution.

However, if the loss function is non-convex, we usually reach the local minima since the gradient is diminishing when reaching the extreme points of the function. This depends on the seed which is used to initiallize the weights of the deep learning model. Therefore, many methods have been proposed to find a better results by overcome the loss function's valleys such as momentum, choosing seeds based on loss function analyzing tasks, etc. 

There are different variations of gradient descent, such as stochastic gradient descent (SGD) and mini-batch gradient descent, which involve updating the parameters based on a subset of the training data instead of the entire dataset. These variations can be more efficient than batch gradient descent, which updates the parameters based on the entire dataset.

\subsubsection{Stochastic Gradient descent}

Stochastic gradient descent (SGD) is a variation of the gradient descent algorithm used in machine learning and deep learning. It is an optimization algorithm that updates the parameters of a model by computing the gradient of the loss function with respect to a randomly selected subset of the training data, rather than using the entire dataset.

In stochastic gradient descent, the model parameters are updated after each iteration, based on the gradient of the loss function with respect to a randomly selected sample of the training data. This means that the gradient is computed on a smaller subset of the data, which can lead to faster convergence and better generalization performance than batch gradient descent. In detail, stochastic gradient descent have the following steps:
\begin{enumerate}
    \item Randomly sample a example $x_i$ from dataset $D$
    \item Compute the loss: $L(w(x_i),y_i)$
    \item Perform gradient descent step $w \leftarrow w \nabla L(w(x_i),y_i)$
    \item Repeat step 1 to 3 till the end of an epoch.
\end{enumerate}

The random sampling of the training data also helps to reduce the risk of the algorithm getting stuck in a local minimum, as it is more likely to escape from a poor local minimum and converge to a better global minimum.

However, the randomness in stochastic gradient descent can introduce some noise into the parameter updates, which can lead to fluctuations in the optimization process. To address this issue, techniques such as learning rate schedules, momentum, and adaptive learning rates are often used in conjunction with stochastic gradient descent to improve its stability and convergence performance.

\subsubsection{Minibatch Stocastic Gradient descent}

In Minibattch Stocastic Gradient Descent, instead of feeding one sample at a time like SGD, we sample a minibatch randomly and execute stocastic gradient descent method on this minibatch. This helps us to speed up the training process compared to SGD and also allows us to train on large dataset.

\begin{enumerate}
    \item Randomly sample a minibatch $B$ from dataset $D$
    \item Compute the losses: $L(w(x_i),y_i)$ for $(x_i,y_1) \in B$
    \item Perform gradient descent step $w \leftarrow w \frac{1}{|B|}(\sum_{i=1}^{|B|}\nabla L(w(x_i),y_i))$
    \item Repeat step 1 to 3 till the end of an epoch.
\end{enumerate}

==> Chapters/03_DPSGD.tex <==
\chapter{Differentially Private Stocastic Gradient Descent}
\label{chapter:DPSGD}

\section{DPSGD}
Abadi \cite{Abadi_2016} has proposed a differentially private training method for minibatch stochatic gradient descent. There is two main steps adding in the training process which are clipping step and add noise step which is shown in the algorithm \ref{alg:DPSGD}.

According to algorithm \ref{alg:DPSGD}, although we sampled mini-batches but we still have to compute per sample's gradients in order to perform clipping step in line 8. This computation is expensive and we can not apply parallelism training of the Deep Learning training frameworks such as Tensorflow or Pytorch. 
\begin{algorithm}[H]
\caption{Differential Private Stochastic Gradient Descent}
\label{alg:DPSGD}
\begin{algorithmic}[1]
 \Procedure{DPSGD}{$d$}
%\Procedure{LocalSGDwithDP}{$d,C,s,\sigma,T$}
\State {\bf Input:} database $D = \{x_1,x_2, \dots, x_n\}$, loss function $\ell(\theta) = \frac{1}{N} \sum_{i} \ell(\theta,x_i)$, learning rate $\eta_t$, noise scale $\sigma$, group size L, gradient norm bound C.
\State {\bf Initialize:} $\theta_0$ randomly.
 
\For {$t \in T$}
    \State Take a random sample $L_t$ with sampling probability $q = L/N$
    \For{$i \in L_t$}
        \State $g_t(x_i) \leftarrow \nabla_{\theta_t} \ell(\theta,x_i)$ \Comment{Compute gradient}
        \State $\bar{g_t}(x_i) \leftarrow g_t(x_i)/ max(1, \frac{||g_t(x_i)||_2}{C})$ \Comment{Clipping Norm}
    \EndFor
    \State $\tilde{g_t} \leftarrow \frac{1}{L} (\sum_{i} \bar{g}_t(x_i) + \mathcal{N}(0,\sigma^2 C^2 I))$  \Comment{Add noise}
    \State $\theta_{t+1} = \theta_{t} - \eta_t \tilde{g_t} $
\EndFor
\State {\bf Output:} $\theta_K$ and compute the overall privacy cost $(\epsilon,\delta)$ using Moment Accountant method.
   
\EndProcedure
\end{algorithmic}
\end{algorithm}



% TODO: write about fast clipping papers?

\subsubsection{Moment Accountant}
The algorithm \ref{alg:DPSGD} is proven to be $(\epsilon,\delta)-DP$ of we choose $\sigma = \Omega(\sqrt{T \log(1/\delta) \log(T/\delta)} /\epsilon)$ where T is the number of iterations. This implies we have to fix 3 in 4 parameters: $T,\sigma , \epsilon, \delta$ before training and we will have limited training iterations.  
Therefore, Abadi \cite{Abadi_2016} also provides Moment Accountant method in order to compute the privacy budget $(\epsilon,\delta)$ after each epoch which means we will fix the number of iterations, $\sigma$ value and one privacy parameter $\epsilon$ or $\delta$ before training. This shows us a limited choice of parameters and it is very hard to find a good settings which helps our neural network have good testing accuracy.

\subsection{f-DP Background}
However, the $(\epsilon,\delta)$-DP definition does not provide a clear measure of a model's privacy level, making it challenging to choose an appropriate privacy budget for DPSGD against strong attacks like Membership Inference Attack\cite{shokri2017membership} and Deep Leakage attacks \cite{zhu2019deep}. Furthermore, in this definition, probabilities rely solely on the randomness of the mechanism ${\cal M}$. Therefore, the level of noise added to the mechanism ${\cal M}$ must be large enough to conceal all characteristics of individual data in dataset $D$. If ${\cal M}$ is a model focused on improving accuracy in specific tasks like image classification, excessive noise can significantly reduce the model's accuracy.

In contrast, Dong et al. \cite{dong2019gaussian} proposed the state-of-the-art Differential Privacy notation, $f$-Differential Privacy, based on hypothesis testing, which is a key idea behind statistical attacks. This framework surpasses all other existing frameworks based on $(\epsilon,\delta)$-DP. Specifically, in hypothesis testing, an adversary attempts to differentiate between two adjacent datasets $D$ and $D'$ based on the output of a differentially private mechanism ${\cal M}$.:

\[H_0: \mbox{The underlying dataset is}\ D\ \mbox{and}\ H_1: \mbox{The underlying dataset is}\ D'\]

Similarly to the $(\epsilon, \delta)$-DP definition, the neighboring datasets are those which differ by only one data row: $|D \cup D'| = 1$. Here, we define Type I and Type II errors as:

\[\alpha_\phi = \mathbb{E}_{o\sim {\cal M}(D)}[\phi(o)]  \mbox{ and } \beta_\phi = 1- \mathbb{E}_{o\sim {\cal M}(D')}[\phi(o)] \]

where $\phi(o) \in [0,1]$ is the rejection rule that takes the output $o$ of the DP mechanism ${\cal M}$ as input. Here, we toss a coin and reject the null hypothesis with probability $\phi$. The optimal trade-off function between Type I and Type II errors is defined as:

\[T({\cal M}(D),{\cal M}(D'))(\alpha) = \inf_\phi \left \{ \beta_\phi : \alpha_\phi \leq \alpha \right\}\]
for $\alpha \in [0,1]$ and the infimum is taken over all measureable rejection rules $\phi$.

If the statistical attack succeeds, it means that the two hypotheses are fully indistinguishable. This leads to the trade-off function $1-\alpha$. A function $f: [0,1] \rightarrow [0,1]$ is a trade-off function if and only if it is convex, continuous, non-increasing, and $f(x) \leq 1-x$ for $x \in [0,1]$. Then, we have the definition of $f$-differential privacy as follows:
\begin{definition}
\label{def:f-DP}
f-differential privacy: Let $f$ be a trade-off function. A mechanism $\cal{M}$ is f-differentially private if
\[T({\cal M}(D), {\cal M}(D')) \geq f\]
for all neighboring datasets $D$ and $D'$
\end{definition}

Moreover, Dong et al. \cite{dong2019gaussian} also defines the Gaussian DP as a special case of $f-DP$ where $f$ is a trade-off function:

\[G_\mu(\alpha) = T({\cal N}(0,1),{\cal N}(\mu,1))(\alpha) = \Phi( \Phi^{-1}(1-\alpha) - \mu) \]
where $\Phi$ is the standard normal cumulative distribution of ${\cal N}(0,1)$. 


Here we have the GDP definition:
\begin{definition}
    A mechanism $\cal M$ is $\mu$- Gaussian Differential Privacy ($\mu$-GDP) if it is $G_{\mu}$-DP:
    \[T({\cal M}(D), {\cal M}(D') \geq G_\mu\]
    for all neighboring dataset $D$ and $D'$
    
\end{definition}

Using the GDP definition, we can easily determine which value of $\mu$ guarantees a reasonable amount of privacy, as shown in Figure 3 (\cite{dong2019gaussian}). For example, $\mu=0.5$ and $\mu=1$ are reasonably private values, while $\mu=3$ or $\mu=6$ are basically non-private because an adversary can control Type I and Type II errors at very small values such as $0.07$ and $0.001$, respectively.

Similar to Abadi et al. \cite{Abadi_2016}, Dong et al. \cite{dong2019gaussian} also prove in Theorem 2.7 that the Gaussian mechanism operating on a statistic $\theta$ as ${\cal M}(D) = \theta(D) + \xi$, where $\xi \sim {\cal N}(0,sens(\theta)^2/\mu^2)$, is $\mu$-GDP. Here, the sensitivity of $\theta$ is defined as:

\[ sens(\theta) = \sup_{D,D'}|\theta(D) - \theta(D')|\]

where the supremum is taken over all neighboring datasets.
Therefore, GDP offers the tightest privacy bound for the Gaussian mechanism.

However, in the case of deep learning where we add Gaussian noise to each layer, we need to compute the composition of the GDPs of all $n$ layers: $\mu = g(\mu_1,\mu_2,\dots,\mu_n)$. Here, let $y_i \leftarrow {\cal M}i(aux,D)$ with $aux = (y_1,...,y{i-1})$, Theorem 3.2 in \cite{dong2019gaussian} shows that if the mechanism ${\cal M}(aux,D)$ is $f_i$-DP for all $aux$, then the $n$-fold composed mechanism $\cal M$, which applies ${\cal M}i$ in the order from $i=1$ to $i=n$, is $(f_1 \otimes f_2 \otimes \dots \otimes f_n)$-DP because the tensor product is commutative. In the special case of the composition of Gaussian operators $G{\mu_i}$, Corollary 3.3 in \cite{dong2019gaussian} states that the $n$-fold composition of $\mu_i$-GDP mechanisms is $\sqrt{\mu_1^2 + \dots + \mu_n^2}$-GDP.

Moreover, if datasets $D$ and $D'$ differ by more than one sample, say $g$ samples where $g>1$, Dong et al. \cite{dong2019gaussian} also show that if a mechanism is $G_{\mu}$-DP for $g=1$, then it is $G_{g\mu}$-DP for groups of size $g$. This is a very nice result because it shows the linear dependency in $g$, and it is a backbone theory for our batch clipping method.



==> Chapters/04_DPSGD_gen.tex <==
\chapter{Generalized Framework for DP-SGD}
\label{chapter:generalizedframeworkDPSGD}
Van Dijk et al. \cite{vandijk2023generalizing} have proposed a generalized framework for DPSGD that allows us to train any machine learning algorithm differentially privately. Moreover, this framework also supports shuffling sampling, which has better performance than subsampling methods \cite{safran2021good}. Therefore, we can use this framework to train our method (shuffling + layerwise batch clipping) without violating privacy. We simplified algorithm 1 in \cite{vandijk2023generalizing}, which is written for the federated learning setting, to a single client training algorithm, shown in Algorithm \ref{alg:genDPSGD}.

In \cite{vandijk2023generalizing}, two sampling methods are analyzed:

\begin{itemize}
    \item Subsampling (SS): In this method, a batch $S_B$ with $|S_B| = sm$ is randomly sampled from the data set $D$ with replacement. Thus, the batches sampled by this method may have intersections. Moreover, this is the sampling method which is used in \cite{Abadi_2016}.
    \item Shuffling (SH): In this method, the whole data set $D$ is shuffled by a random permutation $\pi^e$ and then divided into equally-sized batches $S_b$ with $|S_b| = sm$ in a random way. Therefore, the batches sampled by this method are disjoint, i.e., $D= \cup^{N/(ms)}_{b=1} S_b$.
\end{itemize}
%%%% Shuffling Batch clipping algorithm %%%%%%
\begin{algorithm}[t]
\caption{%Differential Private SGD -- 
Generalized Framework for DP-SGD}
\label{alg:genDPSGD}
\begin{algorithmic}[1]
%\Procedure{LocalSGDwithDP}{$d,C,s,\sigma,T$}
\Procedure{DP-SGD-General}{}
   \State \textbf{Input:} Dataset size $N$,dataset $(D=\{\xi_i\}_{i=1}^{N})$, number of epochs $(E)$, diminishing round step size sequence $\{\eta_i\}_{i=1}^{T}$, the default initial model $(w)$, Gradient clipping value $(C)$, noise scale $\sigma$
    \For{$e\in \{1,\ldots, E\}$}
    \State Let $\pi^e$ be a random permutation 
    \State re-index data samples: $\{\xi_i\leftarrow \xi_{\pi^e(i)}\}_{i=1}^N$  
    \State $\{S_{b,h}\}_{b=1,h=1}^{N/(ms),m}\leftarrow$ ${\tt Sample}_{s,m}$ with $S_{b,h}\subseteq \{1,\ldots, N\}$, 
    \Comment{ $|S_{b,h}|=s$, $|S_b|=sm$ with $S_b=\bigcup_{h=1}^m S_{b,h}$ }
    \For{$b\in \{1,\ldots, \frac{N}{ms}\}$}
%    \State Set $w$ equal to last received global model
 %   \State $U=0$
 \State Start of round $(e-1)\frac{N}{ms}+b$:
    \For{$h\in \{1,\ldots,m\}$}
    \State $a_h\leftarrow {\cal A}(w,\{\xi_i\}_{i\in S_{b,h}})$
    \State $[a_h]_C = a_h/\max(1,\frac{||a_h||_2}{C})$ \Comment{Clipping gradient}
 %   \State $U\leftarrow U+[a]_C$
    \EndFor
    
    \State $U=\sum_{h=1}^m [a_h]_C$
    \State $\bar{U}\leftarrow U+ {\cal N}(0,(2C\sigma)^2{\bf I})$ \Comment{Add Noise}
    \State $w\leftarrow w- \eta_{(e-1)\frac{N}{ms}+b} \cdot \bar{U}/m$
    \EndFor
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

The algorithm ${\cal A}$ could be any optimization algorithm (such as SGD, ADAM, etc.) and only depends on $w$ and the batch of data samples $S_{b,h}$. Moreover, based on the DP analysis in \cite{vandijk2023generalizing}, this generalized framework also enables us to apply batch normalization, where the normalization is performed on the samples in batch $S_{b,h}$. Thus, we can even use a batch normalization layer in our neural network's architecture.

\subsubsection{Clipping}
In algorithm \ref{alg:genDPSGD}, the gradients $a_h$ are clipped as follow:
\[[a_h]_C = a_h/\max(1,\frac{||a_h||_2}{C})\]
and then added into the updated value $U = \sum_{h=1}^m [a_h]_C = \sum_{h=1}^m [a_h/\max(1,\frac{||a_h||_2}{C}]_C$

Note that the batch size $|S_b| = sm$ and the micro-batch size $|S_{b,h}|=s$, allowing us to switch the clipping settings by choosing the appropriate values of $s$ and $m$. Specifically, we have the following options:
\begin{itemize}
    \item Individual Clipping ($s=1$): In this setting, each micro-batch $S_{b,h}$ contains only one sample. As a result, $[a_h]_C$ represents the clipped value of each sample's gradient, leading to an individual clipping setting similar to \cite{Abadi_2016}.
    \item Batch Clipping ($m=1$): With only one micro-batch $S_{b,h}$ that contains all samples in the batch ($S_b = S_{b,h} = s$), the gradient values of the whole batch computed by the optimization algorithm ${\cal A}$ are used for clipping ($a_h$). This approach can leverage parallel computation provided by popular frameworks such as Tensorflow and PyTorch, leading to significantly reduced training time. However, the entire batch's gradients are clipped with the same value $C$, which may result in a higher gradient norm compared to individual clipping, potentially losing more information in the gradients.
    \item Mixing Clipping ($1 < s,m < sm$): Finally, Van Dijk et al. \cite{vandijk2023generalizing} also provides a mixing clipping method where we have $m$ micro-batches with size $s$. This method attempts to combine the benefits of individual and batch clipping methods.
\end{itemize}

However, based on the experimental results presented in \cite{vandijk2023generalizing}, the batch clipping method showed the highest performance for a CNN architecture with 4 convolutional layers. Therefore, we chose to use the batch clipping method to evaluate our new algorithm, which is described in chapter \ref{chapter:layerwiseclipping}.

\subsubsection{DP guarantee}

In \cite{vandijk2023generalizing}, the adversary is stronger compared to the adversary in \cite{dong2019gaussian}. This adversary knows which sampling method was used and how it works. They can derive a joint probability distribution of the number of differentiating data samples for each sampling round within the sequence of rounds. In contrast, the adversary in the $f$-DP analysis \cite{dong2019gaussian} considers each round separately and analyzes a single round. In other words, the adversary in \cite{vandijk2023generalizing} has extra information from the sampling operator by observing the outcome of multiple rounds and can use it to enhance the statistical attack.

Therefore, Van Dijk et al. \cite{vandijk2023generalizing} enables us to use other sampling methods rather than mini-batch SGD, which was introduced in the original DPSGD paper \cite{Abadi_2016}. Applying the $f$-DP terminology, the general algorithmic framework is $G_{\sqrt{gE}/\sigma}$-DP with a $\sqrt{gE}$ dependency, where $g$ is the group size, $E$ is the total number of epochs, and $\sigma$ is the noise multiplier in Gaussian noise.


==> Chapters/05_Normalization.tex <==
\chapter{Normalization}
\label{chapter:Normalization}
\section{Data Normalization}
TODO: Explain why do we need Data Normalization and what it is (Scale off all data to specific range)

TODO: Explain shuffling versus sub sampling
\section{Batch Normalization}
TODO: Explain why Batch Normalization in Deep Learning in good (trainning speed, testing accuracy)

==> Chapters/07_Experiments.tex <==
\section{Experiments}
\label{section:Experiments}

This section reports on our evaluation of the batch clipping method, diminishing clipping value $C$, layerwise clipping values $C_i$, and results on two popular image datasets: MNIST and CIFAR-10. Moreover, we also show that our method outperforms Opacus settings in terms of testing accuracy. The code is available at \href{https://github.com/MisaNguyen/DPSGD/tree/master}{https://github.com/MisaNguyen/DPSGD/tree/master}.

% In order to demonstrate the power of the algorthm (TODO: Cite the algo), we run this algorithm under various optimization methods, deep learning models and hyper-parameters settings. Due to the dataset complexity, we also try out different deep learning model accordingly: Lenet-5, Convolutional Neural Network with 5 convolutional layers, Alex-net, Resnet-18, Resnet-50. More importantly, since we can apply any algorithm to compute the gradients, we also experiments with different model optimizers: Stocastic gradient descent (SGD), ADAM. Moreover, based on the dataset, model architecture and model optimizer we choose, we also do the sensitivity studies on the hyperparameters: Learning rate $\eta$, master clipping norm constant $C$, the Gaussian noise variance scale $\sigma$ and the batch size $|B|$. 
\subsection{Training Configuration}
Testing accuracy depends on various factors such as the batch size $|S_b|$, learning rate $\eta$, clipping norm $C$, Gaussian noise $N(0,(2C\sigma)^2)$, model architecture, number of epochs $E$ or training iterations, data augmentation, data normalization, sampling method, optimizer, and training algorithm. In our experiments, we define a set of parameters to explore how these variables affect testing accuracy. Our objective is to identify the optimal configuration that achieves the highest testing accuracy while keeping the privacy budget $(\epsilon,\delta)$ as small as possible.

To ensure consistency, we apply data augmentation and normalization on the training dataset before feeding the images to the neural network. We also shuffle the entire dataset at the beginning of each epoch before splitting it into training batches. These techniques are used in all of our experiments for the following reasons:

\begin{itemize}
\item Data Augmentation \cite{dataAugpaper}: This technique enhances the size and quality of the training dataset to avoid overfitting and improve the generalization ability of the neural network, which can lead to better testing accuracy.
\item Data Normalization \cite{dataNormpaper}: This technique helps the convolutional neural network learn faster and even improve testing accuracy in some scenarios. Since our experiments involve image classification using convolutional layers in our neural networks, we consider this technique to be helpful.
\item Random Shuffling in each epoch \cite{safran2021good}: This technique has proven to have smaller optimization error than subsampling (where we sample the data batches with replacements) for the SGD optimizer. Therefore, we also applied this technique to enhance our testing accuracy further.
\end{itemize}

Our main goal is to demonstrate the effectiveness of our model when utilizing the batch clipping method, diminishing clipping value, and layerwise clipping during the training process of our differentially private model. Therefore, we conduct four experiments for each dataset using the SGD optimizer and the methods listed in Table \ref{tab:Experiments}:

\begin{table}[ht]

\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
   \multicolumn{2}{|c|}{Sampling} & \multicolumn{2}{|c|}{Clipping method} & \multicolumn{2}{|c|}{Clipping value} & \multicolumn{2}{|c|}{Clipping mode} & \multicolumn{3}{|c|}{Testing Accuracy} & Note\\ \hline 
   SS & SH & BC \qquad & IC & Cons & Dim  & Layer & Full & MNIST& \multicolumn{2}{|c|}{CIFAR10} &\\ \hline
   \multicolumn{8}{|c|}{ } & Lenet-5 & convnet & resnet18 & \\ \hline
   x &   &   & x &   & x &   & x & $89.70\%$&$37.08\%$ & $51,24\%$& Opacus\\ \hline
   & x & x &   & x &   &   & x & $\approx 98\%$  & $\approx 65\%$ & N/A &\cite{vandijk2023generalizing}\\ \hline
   
    & x & x &   & x &   & x &   & $98.25\%$ & $68.54\%$  & $90.78\%$  &ours\\ \hline
   & x & x &   &   & x & x &   & $98.25\%$& $60.31\%$ & $91.06\%$ &ours\\ \hline
 % 4 & &   & x & x &   &   & x &   & x & ours\\ \hline
  
\end{tabular}
}
\caption{Experiments description: SS and SH stand for subsampling and shuffling. "BC" and "IC" are the batch clipping and individual clipping methods, respectively. "Cons" and "Dim" refer to the constant and diminishing clipping values. "Layer" and "Full" indicate whether we clipped the gradient at each layer or fully clipped the parameters of the entire model. The testing accuracy is achieved after 50 training epochs with a diminishing learning rate $\eta$ and different Gaussian noise multipliers $\sigma$, batch sizes $S_b$, and clipping values $C$ described in Table \ref{tab:hyperparameter}. with a privacy budget of $(\epsilon,\delta) = (1,1/N)$, where $N$ is the size of the training dataset. The testing accuracy is the best testing accuracy for $\sigma = 2$ where we have the same privacy $G_{\sqrt{gEL/}\sigma}$}
\label{tab:Experiments}
\end{table}
We do the experiments on the parameters defined in Table \ref{tab:hyperparameter}. Besides, for diminishing learning rate $\eta$ and clipping value $C$, we update these two parameter after each training epoch:
\[\eta = \eta \times \eta_{decay}\]
And
\[C = C \times C_{decay} \textit{\ in\ diminishing\ clipping\ value\ case}\] 
\begin{table}[ht]

\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|}
\hline
 Learning Rate $\eta$ & $0.025$ \\ \hline 
 Clipping value ($C$) & $[0.005,0.01,0.05,0.1,0.5,1.0]$ \\ \hline 
 $\sigma$ & $[2,4,8]$ \\ \hline 
 Learning rate decay ($\eta_{decay})$ & $0.9$ \\ \hline 
 Clipping value decay ($C_{decay}$) & $0.9$ \\ \hline 
 Batch size ($|S_b|$) & $[64,128,256,512,1028]$\\ \hline 
\end{tabular}
}
\caption{Hyperparameter settings}
\label{tab:hyperparameter}
\end{table}

For the layerwise clipping method, we compute the clipping value for each layer based on the gradient ratio between each layer. Therefore, these clipping values will leak information about the training data if the gradient ratio is computed based on the training data. To address this issue, we randomly split the training dataset $D$ into two subsets:

\begin{itemize}
    \item Subset for training the neural network $D_{train}$: We use this subset to train the neural network model and optimize the model based on the examples in it.
    \item Subset for computing gradient ratios $D_{dummy}$: We use this subset to compute the ratio of gradients by simply inputting it to the current model at a certain epoch and then computing the gradients. Note that we do not update the model using these gradients. In the case of diminishing clipping value $C$, we recompute the clipping value of each layer whenever we update a new value $C$.
\end{itemize}

In our experiments, the size of the training data $|D_{train}|$ is $\frac{9}{10}|D|$, and the size of the dummy data $|D_{dummy}|$ is $\frac{|D|}{10}$.
\subsection{Opacus comparison}
We want to run Opacus and our algorithm under the same privacy and then compare the performance based on the testing accuracy after 50 training epochs.

Since our algorithm \ref{alg:layerwiseDPSGD} is prove to be $G_{\sqrt{gEL}/\sigma}$, we choose the same noise added in the Opacus setting: $\bar{\sigma} = \sigma / \sqrt{L}$. For example, in resnet18 model, there are total 62 layers which have gradients where we add the Gaussian noise. Thus, $\bar{\sigma} = \sigma/\sqrt{62}$.

\textbf{Combining constant clipping value with layerwise batch clipping method:}
In this method, we do not decrease the clipping value $C$ and we only compute the layerwise clipping values $c_i$ for $i$-th layer once before training the model. After running a wide range of $C$, we are able to achieve the closest performance compared to the baseline result. Specifically, we achieved $98.25\%$,$98.07\%$, $97.68\%$ with $\sigma = 2,4,8$ and $C = 0.005$, respectively. This means given a good clipping value $C$, we can use larger Gaussian noise multiplier $\sigma$ without hurting the model's testing accuracy too much. This yields stronger privacy $G_{\sqrt{gEL}/\sigma}$-DP as $\sigma$ increases. However, finding this $C$ value maybe a hard task and it is heavily dependent on the each gradient value in each neuron in the model. The results are shown in figures \ref{fig:MNISTAccuracy_BC_CCV_L} and \ref{fig:CIFAR10Accuracy_BC_CCV_L}

\textbf{Combining diminishing clipping value with layerwise batch clipping method:}
In this experiments, we use the diminishing clipping value which starts with $C$ and then recomputes the layerwise clipping values $c_i$ whenever we update the new $C$. We also achieve the similar results compared with constant clipping value method. This implies that the value $C$ can move along with the trends of gradients without hurting the model's testing accuracy. However, we could not see the different in performance between two methods with MNIST dataset and Lenet-5 model which are the simple dataset and model architecture. The results are shown in figures \ref{fig:MNISTAccuracy_BC_DCV_L} and \ref{fig:CIFAR10Accuracy_BC_CCV_L}

\subsection{MNIST}
   Firstly, we ran our algorithm on a simple dataset, MNIST, which consists of 60,000 training examples and 10,000 testing examples of handwritten digits \cite{Lenet5model}. Each example is a 28x28 gray-level image. For this dataset, we used the LeNet-5 model \cite{Lenet5model}, which has 3 convolutional layers, 2 averaging layers, and 2 fully connected layers. The details of the LeNet-5 architecture are described in Table \ref{tab:Lenet5}. For each training image, we cropped a $32\times32$ image with padding of 4 from it, randomly horizontally flipped the image, and then normalized it with $(mean, std) = ((0.1307,), (0.3081,))$. In our experiments, data augmentation and data normalization were performed independently in each epoch.

\begin{table}[ht]

\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 Operation Layer & \#Filters  & Kernel size & Stride & Padding & Output size & Activation function \\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$ \vspace{1mm}}& $6$ & $5 \times 5$ & $1 \times 1$ & $0$ & $28 \times 28 \times 6$ & $tanh$\\ \hline 
 $AvgPool2d$&   & $2 \times 2$ & $2 \times 2$ &  & $14 \times 14 \times 6$ & \\ \hline 
\parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$\vspace{1mm}}& $16$ & $5 \times 5$ & $1 \times 1$ & $0$ & $10 \times 10 \times 16$ & $tanh$\\ \hline 
 $AvgPool2d$&   & $2 \times 2$ & $2 \times 2$ & &  $10 \times 10 \times 16$ &\\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$\vspace{1mm} }& $120$ & $5 \times 5$ & $1 \times 1$ & $0$ &  $5 \times 5 \times 16$ & $tanh$\\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $FC1$\vspace{1mm} }& $-$ & $-$ & $-$ & $-$ & $84$ & $tanh$\\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $FC2$\vspace{1mm} }& $-$ & $-$ & $-$ & $-$ & $10$ & $softmax$\\ \hline 
\end{tabular}
}
\caption{Lenet-5 model architecture}
\label{tab:Lenet5}
\end{table}

\textbf{Baseline result:}
With our algorithm \ref{alg:layerwiseDPSGD}, we achieved  $98.09\%$ testing accuracy with cross-entropy loss and batch size $|S_b| = 64$ which is consistent with what have shown in \cite{Lenet5model}. 
\begin{figure*}[th!]
\centering
%--------------non-private, SS, MNIST------------------%
\subfigure[LeNet baseline]{\includegraphics[width=0.99\textwidth]{Figs/MNIST/non_private/Lenet_shuffling_SGD_lr_0.025_C_0.1_sigma_2_0.png}}
\caption{MNIST testing accuracy baseline for batch size $|S_b|= sm= 64,128,256,512$ }
\label{fig:MNISTAccuracy}
\end{figure*}

\textbf{Opacus result:}
For MNIST dataset, we observed a slightly decrease in accuracy when we choose $\sigma = 2,4,8$, respectively. In other words, we run the experiments using Opacus framework with $\bar{\sigma} = \sigma/\sqrt{L} = \bar{\sigma} = \sigma/\sqrt{10}$ (Note that convolution layer and fully connected layer has bias values and they also have the gradient, we count each bias as one layer as well) where $\sigma = 2,4,8$ and achieved the testing accuracy of $89.7\%, 87.67\%$ and $83.74\%$. We can clearly see that the testing accuracy is decrease significantly if we try to increase $\sigma$ which yields better privacy. The result of these experiments are shown in figure \ref{fig:OpacusMNIST}
\begin{figure*}[th!]
\centering
%--------------OPACUS, SS MNIST------------------%
\subfigure[$\sigma = 2.0$, top acc = $89.70\%$]{\includegraphics[width=0.32\textwidth]{Figs/MNIST/opacus/LeNet_2.0.png}}
\subfigure[$\sigma = 4.0$, top acc = $87.67\%$]{\includegraphics[width=0.32\textwidth]{Figs/MNIST/opacus/LeNet_4.0.png}}
\subfigure[$\sigma = 8.0$, top acc = $83.75\%$]{\includegraphics[width=0.32\textwidth]{Figs/MNIST/opacus/LeNet_8.0.png}}
\caption{Opacus's spent privacy budget and testing accuracy for MNIST dataset with batch size $|S_b|= sm= 64,128,256,512$ after 50 training epochs}
\label{fig:OpacusMNIST}

\end{figure*}

\textbf{Layerwise Clipping with constant clipping value result:}
On the other hand, with the same privacy where $\sigma = 2,4,8$, we achieved the testing accuracy $98.25\%, 98.09\%, 97.63\%$, respectively. This is the best testing accuracy which reaches the performance of the baseline model where no noise is added. Moreover, the accuracy is maintained while increasing the $\sigma$ value if we could find a suitable clipping value $C$
\begin{figure*}[th!]
\centering
%--------------BC + CCV + Layerwise, MNIST------------------%
%--------------Lenet------------------%
\subfigure[Lenet-5,$\sigma=2$, top acc = $98.25\%$]{\includegraphics[width=0.32\textwidth] {Figs/MNIST/batch_clipping/layerwise/CCV/Lenet_shuffling_BC_lr_0.025_C_0.005_sigma_2_0.png}}
\subfigure[Lenet-5,$\sigma=4$, top acc = $98.07\%$]{\includegraphics[width=0.32\textwidth] {Figs/MNIST/batch_clipping/layerwise/CCV/Lenet_shuffling_BC_lr_0.025_C_0.005_sigma_4_3.png}}
\subfigure[Lenet-5,$\sigma=8$, top acc = $97.68\%$]{\includegraphics[width=0.32\textwidth] {Figs/MNIST/batch_clipping/layerwise/CCV/Lenet_shuffling_BC_lr_0.025_C_0.005_sigma_8_6.png}}
\caption{MNIST testing accuracy with batch clipping + Constant clipping value + layerwise clipping method, }
\label{fig:MNISTAccuracy_BC_CCV_L}
\end{figure*}

\textbf{Layerwise Clipping with diminishing clipping value result:}
As explained in previous chapters, this method has the similar idea as diminishing step size. We would want to decrease the clipping norm since the gradients tends to be smaller when reaching the optimal point.
Our results also show that this method can also reach the performance of the base line model: We achieved the testing accuracy of $98.25\%,98.09\%$ and $97.63\%$ for $\sigma = 2,4,8$, respectively. However, we hardly see the different between diminishing clipping value and constant clipping value methods. Therefore, we decided to run our algorithm on more complex dataset and model architectures.
\begin{figure*}[th!]
\centering
%--------------BC + DCV + Layerwise, MNIST------------------%
%--------------Lenet------------------%
\subfigure[Lenet-5, $\sigma=2$, top acc = $98.25\%$] {\includegraphics[width=0.32\textwidth] {Figs/MNIST/batch_clipping/layerwise/DCV/Lenet_shuffling_BC_lr_0.025_C_0.005_sigma_2_0.png}} 
\subfigure[Lenet-5, $\sigma=4$, top acc = $98.09\%$]{\includegraphics[width=0.32\textwidth] {Figs/MNIST/batch_clipping/layerwise/DCV/Lenet_shuffling_BC_lr_0.025_C_0.005_sigma_4_3.png}} 
\subfigure[Lenet-5, $\sigma=8$, top acc = $97.63\%$]{\includegraphics[width=0.32\textwidth] {Figs/MNIST/batch_clipping/layerwise/DCV/Lenet_shuffling_BC_lr_0.025_C_0.005_sigma_8_6.png}} % 68.82

\caption{MNIST testing accuracy with batch clipping + Diminishing clipping value + layerwise clipping method. }
\label{fig:MNISTAccuracy_BC_DCV_L}
\end{figure*}


%%%%%%%%%%%%%%----------------------------------------%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{CIFAR10}

We conduct similar experiments on the CIFAR-10 dataset as we did on the MNIST dataset. The CIFAR-10 dataset consists of 50,000 training examples and 10,000 test examples, divided into 10 classes, with each example being a 32x32 image with three color channels (RGB) \cite{CIFAR10dataset}. For this dataset, we trained two different models: a convnet with four convolutional layer blocks (each consisting of a convolutional layer with ReLU activation function, followed by an average pool layer with a kernel size of 2x2 and stride value of 2) and one softmax layer, and a ResNet18 \cite{resnet18paper}. We wanted to explore how our method works with both simple and very deep model architectures that have shortcuts, since our work heavily depends on the model architecture with the layerwise clipping method. The details of the convnet and ResNet-18 model architectures are described in Tables \ref{tab:convnet} and \ref{tab:resnet18}, respectively.

For each training image, we crop a $32 \times 32$ region from it with padding of 4, apply a random horizontal flip to the image, and then normalize it with 
\[(mean,std) = ((0.4914, 0.4822, 0.4465), (0.2023,0.1994, 0.2010))\]. In our experiments, we perform data augmentation and data normalization independently in each epoch.
\begin{table}[ht]

\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 Operation Layer & \#Filters  & Kernel size & Stride & Padding & Output size & Activation function \\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$ \vspace{1mm}}& $32$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$ & \multirow[c]{2}{*}{$16 \times 16 \times 3$} & ReLu\\ 
 $AvgPool2d$&   & $2 \times 2$ & $2 \times 2$ &  &  & \\ \hline 
\parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$\vspace{1mm}}& $64$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$ & \multirow[c]{2}{*}{$8 \times 8 \times 32$} & ReLu\\ 
 $AvgPool2d$&   & $2 \times 2$ & $2 \times 2$ &  &  & \\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$\vspace{1mm} }& $64$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$ & \multirow[c]{2}{*}{$4 \times 4 \times 64$} & ReLu\\  
 $AvgPool2d$&  & $2 \times 2$ & $2 \times 2$ &  &  & \\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$ \vspace{1mm}}& $128$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$ & \multirow[c]{2}{*}{$1 \times 1 \times 128$} & ReLu\\ 
 $AdaptiveAvgPool2d$&   & $1 \times 1$ & $1 \times 1$ &    &  & \\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $FC2$\vspace{1mm} }& $-$ & $-$ & $-$ & $-$ & $10$ & $softmax$\\ \hline 
\end{tabular}
}
\caption{convnet model architecture}
\label{tab:convnet}
\end{table}


\begin{table}[ht]

\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 Operation Layer & \#Filters  & Kernel size & Stride & Padding & Output size & Activation function \\ \hline 
 \parbox[c]{3cm}{\vspace{1mm} \centering $Conv2D$ \vspace{1mm}}& $64$ & $7 \times 7$ & $2 \times 2$ & $1 \times 1$ & \multirow[c]{1}{*}{$112 \times 112 $} & ReLu\\ \hline
 $MaxPool2d$&   & $3 \times 3$ & $2 \times 2$ &  &  \multirow[c]{2}{*}{$56 \times 56$} & \\  
 \parbox[c]{5cm}{\vspace{1mm} \centering $2 \times (Conv2D + BatchNorm)$ \vspace{1mm}}& $64$ & $3 \times 3$ & $1 \times 1$ & $1 \times 1$ &  & ReLu\\ \hline
 
 \parbox[c]{5cm}{\vspace{1mm} \centering $2 \times (Conv2D + BatchNorm)$ \vspace{1mm}}& $128$ & $3 \times 3$ & $2 \times 2$ & $1 \times 1$ & $28 \times 28$ & ReLu\\ \hline
 \parbox[c]{5cm}{\vspace{1mm} \centering $2 \times (Conv2D + BatchNorm)$ \vspace{1mm}}& $256$ & $3 \times 3$ & $2 \times 2$ & $1 \times 1$ & $14 \times 14$ & ReLu\\ \hline
 \parbox[c]{5cm}{\vspace{1mm} \centering $2 \times (Conv2D + BatchNorm)$ \vspace{1mm}}& $512$ & $3 \times 3$ & $2 \times 2$ & $1 \times 1$ & $7 \times 7$ & ReLu\\ \hline
 $AvgPool$2D&   & $4 \times 4$ &  &    & \multirow[c]{3}{*}{$1 \times 1$} & \\ 
 \parbox[c]{3cm}{\vspace{1mm} \centering $1000-d\ FC1$\vspace{1mm} }& $-$ & $-$ & $-$ & $-$ &  & \\ 
 \parbox[c]{3cm}{\vspace{1mm} \centering $FC2$\vspace{1mm} }& $-$ & $-$ & $-$ & $-$ &  & $softmax$\\ \hline 
\end{tabular}
}
\caption{resnet18 model architecture}
\label{tab:resnet18}
\end{table}

\textbf{Baseline result: }For non-private training, we achieve \textbf{$69.93\%$} and \textbf{$89.57\%$} testing accuracy respectively for convnet and resnet18 with  batch size $64$ and SGD optimizer for our baseline result.

\begin{figure*}[th!]
\centering
%--------------non-private, SS, CIFAR10------------------%
\subfigure[convnet]{\includegraphics[width=0.49\textwidth]{Figs/CIFAR10/non_private/convnet_shuffling_SGD_lr_0.025.png}}
\subfigure[resnet18]{\includegraphics[width=0.49\textwidth]{Figs/CIFAR10/non_private/resnet18_shuffling_SGD_lr_0.025_C_0.1_sigma_2_0.png}}

\caption{CIFAR10 testing accuracy baseline for batch size $|S_b|= sm= 64,128,256,512$ }
\label{fig:CIFAR10Accuracy}
\end{figure*}

\textbf{Opacus result:}
For CIFAR10, we can see that the model testing accuracy is very bad for convnet and resnet18 models. After 50 training epochs, we can only achieve $\approx 38\%$ and $\approx 48\%$ testing accuracy for convnet and resnet models when choosing $\sigma = 2,4,8$. Here, we have 
$L_{convnet} = 10$ and $L_{resnet} = 62$ and we run the experiments with $\bar{\sigma} = \sigma/\sqrt{L_{convnet}}$  and $\bar{\sigma} = \sigma/\sqrt{L_{resnet}}$ with Opacus framework. The detail of results shown in figure \ref{fig:OpacusCIFAR10}
\begin{figure*}[th!]
\centering
%--------------OPACUS, SS CIFAR10------------------%
%--------------CONVNET------------------%
\subfigure[convnet, $\sigma=2$, top acc = $37.08\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/opacus/convnet_2.0.png}}
\subfigure[convnet, $\sigma=4$, top acc = $39.47\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/opacus/convnet_4.0.png}}
\subfigure[convnet, $\sigma=8$, top acc = $38.78\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/opacus/convnet_8.0.png}}
%--------------RESNET18------------------%
\subfigure[resnet18,$\sigma = 2.0$, top acc = $51,24\%$]{\includegraphics[width=0.32\textwidth]{Figs/CIFAR10/opacus/resnet18_2.0.png}}
\subfigure[resnet18,$\sigma = 4.0$, top acc = $47,46\%$]{\includegraphics[width=0.32\textwidth]{Figs/CIFAR10/opacus/resnet18_4.0.png}}
\subfigure[resnet18,$\sigma = 8.0$, top acc = $43.42\%$]{\includegraphics[width=0.32\textwidth]{Figs/CIFAR10/opacus/resnet18_8.0.png}}
\caption{Opacus's spent privacy budget and testing accuracy for CIFAR10 dataset with batch size $|S_b|= sm= 64,128,256,512$ after 50 training epochs}
\label{fig:OpacusCIFAR10}
\end{figure*}
% We achieve around $\%$, $\%$, $\%$ accuracy with non-private baseline, DP with batch clipping method, DP with batch clipping and diminishing layerwise clipping constant $C_i$ for 50 epochs with batch size of $xxx$ examples; respectively

\textbf{Layerwise Clipping with constant clipping value result:}
As shown in Figure \ref{fig:CIFAR10Accuracy_BC_CCV_L}, the testing accuracy lines are fluctuating more than the Opacus's algorithm. However, although this effects show that complex models are very sensitive with our methods, our algorithm still converge to a good accuracy which can even reach the baseline accuracy. Specifically, we achieve $\approx 68\%$ and $\approx 90.7\%$ testing accuracy for CIFAR10 with convnet and resnet18 models with only 50 training epochs. Similarly to MNIST experiments, even with complex models, our methods still be able to adjust wide range of $\sigma$ value while maintaining the performance. In \cite{vandijk2023generalizing}, we do not have the experiment results for CIFAR10 + resnet18, therefore, we put the $N/A$ value in that cell.
\begin{figure*}[th!]
\centering
%--------------BC + CCV + Layerwise, CIFAR10------------------%
%--------------CONVNET------------------%
\subfigure[convnet, $\sigma=2$, top acc = $68.54\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/CCV/convnet_shuffling_BC_lr_0.025_C_0.005_sigma_2_0}} % 68.65
\subfigure[convnet, $\sigma=4$, top acc = $68.52\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/CCV/convnet_shuffling_BC_lr_0.025_C_0.005_sigma_4_3.png}} % 68.78
\subfigure[convnet, $\sigma=8$, top acc = $61.57\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/CCV/convnet_shuffling_BC_lr_0.025_C_0.005_sigma_8_6}}  % 69.03
%--------------RESNET18------------------%
\subfigure[resnet18, $\sigma=2$, top acc = $90.78 \%$ ]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/CCV/resnet18_shuffling_BC_lr_0.025_C_0.005_sigma_2_0.png}}  
\subfigure[resnet18, $\sigma=4$, top acc = $90.97 \%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/CCV/resnet18_shuffling_BC_lr_0.025_C_0.005_sigma_4_3.png}}  
\subfigure[resnet18, $\sigma=8$, top acc = $90.73 \%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/CCV/resnet18_shuffling_BC_lr_0.025_C_0.01_sigma_8_6.png}}  
\caption{CIFAR10 testing accuracy with batch clipping + Constant clipping value + layerwise clipping method, }
\label{fig:CIFAR10Accuracy_BC_CCV_L}
\end{figure*}

\textbf{Layerwise Clipping with diminishing clipping value result:}
We also try out of diminishing clipping value experiments performs compared to constant clipping value experiments. We observe that the testing accuracy curves becomes smoother and the fluctuation decreased significantly. However, The resnet18 model has the same testing accuracy while convnet model's testing accuracy dropped $\approx 8\%$ down when we switch from constant clipping value mode to diminishing clipping value mode. This implies that this method performs better with deeper neural networks.
\begin{figure*}[th!]
\centering
%--------------BC + DCV + Layerwise, CIFAR10------------------%
%--------------CONVNET------------------%
\subfigure[convnet, $\sigma=2$, top acc = $60.31\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/DCV/convnet_shuffling_BC_lr_0.025_C_0.005_sigma_2_0.png}} % 68.45
\subfigure[convnet, $\sigma=4$, top acc = $60.22\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/DCV/convnet_shuffling_BC_lr_0.025_C_0.005_sigma_4_3.png}} % 68.53
\subfigure[convnet, $\sigma=8$, top acc = $61.43\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/DCV/convnet_shuffling_BC_lr_0.025_C_0.005_sigma_8_6.png}} % 68.82
% %--------------RESNET18------------------%
\subfigure[resnet18, $\sigma=2$, top acc = $91.06\%$]{\includegraphics[width=0.32\textwidth] {Figs/CIFAR10/batch_clipping/layerwise/DCV/resnet18_shuffling_BC_lr_0.025_C_0.005_sigma_2_0.png}} % 90.5
\subfigure[resnet18, $\sigma=4$, top acc = $90.48\%$]{\includegraphics[width=0.32\textwidth]{Figs/CIFAR10/batch_clipping/layerwise/DCV/resnet18_shuffling_BC_lr_0.025_C_0.005_sigma_4_3.png}} % 90.7
\subfigure[resnet18, $\sigma=8$, top acc = $90.99\%$]{\includegraphics[width=0.32\textwidth]{Figs/CIFAR10/batch_clipping/layerwise/DCV/resnet18_shuffling_BC_lr_0.025_C_0.005_sigma_8_6.png}} % 89.5

\caption{CIFAR10 testing accuracy with batch clipping + diminishing clipping value + layerwise clipping method. For resnet18 model, With batch size 64, we achieved $91.06\%$, $90.24\%$ and $90.76\%$ testing accuracy with $\sigma =2,4,8$ respectively.}
\label{fig:CIFAR10Accuracy_BC_DCV_L}
\end{figure*}

\section{Conclusion}
\label{sec:conclusion}
In this paper, we propose a new clipping method which unlock the power of DPSGD. 




